Automated MeSH Term Suggestion for Effective Query Formulation in Systematic Reviews Literature Search

High-quality medical systematic reviews require comprehensive literature searches to ensure the recommendations and outcomes are sufficiently reliable. Indeed, searching for relevant medical literature is a key phase in constructing systematic reviews and often involves domain (medical researchers) and search (information specialists) experts in developing the search queries. Queries in this context are highly complex, based on Boolean logic, include free-text terms and index terms from standardised terminologies (e.g., the Medical Subject Headings (MeSH) thesaurus), and are difficult and time-consuming to build. The use of MeSH terms, in particular, has been shown to improve the quality of the search results. However, identifying the correct MeSH terms to include in a query is difficult: information experts are often unfamiliar with the MeSH database and unsure about the appropriateness of MeSH terms for a query. Naturally, the full value of the MeSH terminology is often not fully exploited. This article investigates methods to suggest MeSH terms based on an initial Boolean query that includes only free-text terms. In this context, we devise lexical and pre-trained language models based methods. These methods promise to automatically identify highly effective MeSH terms for inclusion in a systematic review query. Our study contributes an empirical evaluation of several MeSH term suggestion methods. We further contribute an extensive analysis of MeSH term suggestions for each method and how these suggestions impact the effectiveness of Boolean queries.

==> Theory_and_calculation.tex <==
\section{Theory/calculation}


\subsection{Experimental Setup}
	
	
We use topics from the CLEF TAR task from 2017, 2018, and 2019 \cite{kanoulas2017clef, kanoulas2018clef, kanoulas2019clef}. 15 topics are discarded due to lack of MeSH terms (\textbf{2017}: CD007427, CD010771, CD010772, CD010775, CD010783, CD010860, CD011145; \textbf{2018}: CD007427, CD009263, CD009694; \textbf{2019}: CD006715, CD007427, CD009263, CD009694, CD011768). An additional 1 topic is discarded because of retrieval issues (\textbf{2017}: CD010276), likely resulting from the fact that some queries are automatically translated from queries in one format (Ovid Medline) into another format (PubMed). In total we used 245 topics across all three datasets (116 unique, as each year has partial overlap). For each topic, we divide the Boolean query for that topic into several query fragments. We create these fragments using the transmute tool~\cite{scells2018querylab}. Each fragment contains at least one MeSH term. This results in a total of 311 unique query fragments for the three years (2.68 fragments per query on average). For each of the query fragments, we corrected any errors (e.g., spelling mistakes, syntactic errors), extracted MeSH terms, keywords, query fragment with MeSH terms, and query fragments without MeSH terms. 
%Table~\ref{table:dataset} presents statistics about the query fragments. 
For training the LTR model for MeSH term ranking, the pre-split training and test portions from the CLEF datasets are used. The 2019 topics are split also on systematic review type (intervention and diagnostic test accuracy --- indicated as `intervention' and `dta' respectively in the results), while those for 2017 and 2018 are all diagnostic test accuracy. We use the quickrank library~\cite{capannini2016quality} for LTR, instantiated with LambdaMART trained to maximise nDCG. We leave other settings as per default.
	
